Efficient Numerical Optimal Control for Highly Oscillatory Systems

We present an efficient transcription method for highly oscillatory optimal control problems. For these problems, the optimal state trajectory consists of fast oscillations that change slowly over the time horizon. Out of a large number of oscillations, we only simulate a subset to approximate the slow change by constructing a semi-explicit differential-algebraic equation that can be integrated with integration steps much larger than one period. For the solution of optimal control problems with direct methods, we provide a way to parametrize and regularize the controls. Finally, we utilize the method to find a fuel-optimal orbit transfer of a low-thrust satellite. Using the novel method, we reduce the size of the resulting nonlinear program by more than one order of magnitude.

==> sections/background.tex <==
\section{Background}

Over the past decades a number of methods have been developed for the treatment of highly oscillatory systems...
This approach is closely related to the \textit{stroboscopic method for highly oscillatory problems} \cite{Calvo2012} and the \textit{heterogeneous multiscale method} \cite{Ariel2013} where the envelope dynamics are also modeled with a differential equation and then numerically approximated. 
Quite similar as well are the \textit{multirevolution methods}\cite{MaceThomas1960,Graf1972} and the \textit{envelope following methods} \cite{Petzold,petzold_jay_yen_1997,Graf1972,Gallivan1980} that instead of approximating the continuous system \eqref{eq:envelopeDynamics}, construct a difference equation that captures the slow changes in the series of periodic points.

% Finding the period of an oscillatory system using numerical methods has been the subject of papers like \cite{Dednam2014}. 
% In the paper, they solve the minimization problem
% \begin{align}
%     \min_T \|R(T)\|^2_2 && R =  \begin{bmatrix}
%         x(T) - x(0)\\ x(T+\Delta t) - x(\Delta t) \\ \vdots 
%     \end{bmatrix}
% \end{align} 
% using Newton-type methods to find the period \(T\) of the system. This is a 'discrete version' of the idea of \cite{Petzold}, where they, in the subject of envelope following methods, proposed minimizing
% \begin{align}
%     \min_{T} \int_0^{T'} (x(t + T) - x(t))^2 \dd t
% \end{align}
% to find the period duration \(T\) from an approximation \(T'\) \cite{Petzold}. 
% The detection of periodic behavior has also been discussed in \cite{Gear1982}, where they find periodic points by evaluating the zero-crossing of the derivative of the trajectory. 
% But since ``anything but a simple periodic solution may lead to more than one zero-crossing in a single period'', they also evaluate the norm of the difference of the derivatives of two considered points \cite{Gear1982}. 
